A Unified System for Data Analytics and In Situ Query Processing

In today's world data is being generated at a high rate due to which it has become inevitable to analyze and quickly get results from this data. Most of the relational databases primarily support SQL querying with a limited support for complex data analysis. Due to this reason, data scientists have no other option, but to use a different system for complex data analysis. Due to this, data science frameworks are in huge demand. But to use such a framework, all the data needs to be loaded into it. This requires significant data movement across multiple systems, which can be expensive. We believe that it has become the need of the hour to come up with a single system which can perform both data analysis tasks and SQL querying. This will save the data scientists from the expensive data transfer operation across systems. In our work, we present DaskDB, a system built over the Python's Dask framework, which is a scalable data science system having support for both data analytics and in situ SQL query processing over heterogeneous data sources. DaskDB supports invoking any Python APIs as User-Defined Functions (UDF) over SQL queries. So, it can be easily integrated with most existing Python data science applications, without modifying the existing code. Since joining two relations is a very vital but expensive operation, so a novel distributed learned index is also introduced to improve the join performance. Our experimental evaluation demonstrates that DaskDB significantly outperforms existing systems.

==> datasets.tex <==
\begin{table}
\caption{Dataset Distributions}
\vspace{-0.23cm}
\label{tab:dataspecs}
\begin{tabular}{lp{3.2cm}l}
\toprule
\textbf{Abbreviation} & \textbf{Description} & \textbf{Cardinality}\\
\midrule
Rseq & Repeating Sequential & Deterministic\\[2pt]
Rseq-Shf & Rseq Uniform Shuffled & Deterministic\\[2pt]
%\hline
Hhit & Heavy Hitter & Deterministic\\[2pt]
Hhit-Shf & Hhit Uniformly Shuffled & Deterministic\\[2pt]
%HHit-Shf & \makecell[tl]{Heavy Hitter\\ Shuffled} & Deterministic\\[2pt]
%\hline
Zipf & Zipfian & Probabilistic\\[2pt]
%\hline
MovC & Moving Cluster & Probabilistic\\[2pt]
\bottomrule
\end{tabular}
\vspace{-0.15cm}
\end{table}
\vspace{-0.15cm}
\section{Datasets}
\label{sec:datasets}

In order to effectively evaluate the algorithms, we generate a set of synthetic datasets that vary in terms of input size, group-by cardinality, key distribution, and key range. %We operate on fixed-length 32-bit integers in the form of key-value pairs. %This is common for many aggregation workloads, as the widest numeric attribute in popular TPC-H benchmark can actually be encoded in 24 bits \cite{council2017tpc}, and many other popular data types can be encoded as integers. Furthermore, the number of entries in a table is typically less than $2^{32}$ \cite{kim2009sort}. 
Our datasets are based on the highly popular input distributions described in prior works \cite{gray1994quickly, cieslewicz2007adaptive, jiang2017efficient}. We employ several tweaks to these datasets, with the goal of expanding the data characteristics that we evaluate. Some datasets, such as the sequential dataset, produce very predictable patterns. For such datasets, we generate an additional variant with uniform random shuffling. In \cite{cieslewicz2007adaptive} it is mentioned that the group-by cardinality is often probabilistic. We enforce deterministic group-by cardinality in cases where the target distribution of the dataset would not be affected. 

%\begin{tabular}{p{2.0cm}p{3.0cm}p{2.5cm}}
%\begin{tabular}{cccc}



% \begin{table}
% \caption{Dataset Distributions}
% \label{tab:dataspecs}
% \begin{tabular}{|c|c|c|c|}
% \hline
% \textbf{Abbreviation} & \textbf{Full Name} & \textbf{Cardinality}\\
% \hline
% RSeq & Repeating Sequential & Deterministic\\
% \hline
% RSeq-Shf & \makecell{Repeating Sequential\\Shuffled} & Deterministic\\
% \hline
% HHit & Heavy Hitter & Deterministic\\
% \hline
% HHit-Shf & \makecell{Heavy Hitter \\Shuffled} & Deterministic\\
% \hline
% Zipf & Zipfian & Probabilistic\\
% \hline
% MovC & Moving Cluster & Probabilistic\\
% \hline
% \end{tabular}
% \end{table}

Throughout this paper we use \textit{random} to refer to a uniform random function with a fixed seed, and \textit{shuffling} refers to the use of the aforementioned function to shuffle all the records in a dataset. The number of records in the dataset is denoted as \textit{r} records and the group-by cardinality is \textit{c}.

In the repeating sequential dataset (\textit{RSeq}), we generate a series of segments that contain number sequences. The number of segments is equal to the group-by cardinality, and the number of records in each segment is equal to the dataset size divided by the cardinality. A shuffled variant of the repeating sequential dataset (\textit{RSeq-Shf}) is also generated. This dataset mimics transactional data where the key incrementally increases.

In the heavy hitter dataset (\textit{HHit}), a random key from the key range accounts for $50\%$ of the total keys. The remaining keys are produced at least once to satisfy the group-by cardinality, and then chosen on a random basis. In a variant of this dataset, the resulting records are shuffled so that the heavy hitters are not concentrated in the first half of the dataset. Real world examples of heavy hitters include top selling products, and network nodes with the highest traffic.

In the Zipfian dataset (\textit{Zipf}), the distribution of the keys is skewed using Zipf's law \cite{powers1998applications}. According to Zipf's law, the frequency of each key is inversely proportional to its rank. We first generate a Zipfian sequence with the desired cardinality $c$ and Zipf exponent $e=0.5$. Then we take $r$ random samples from this sequence to build $r$ records. The final group-by cardinality is non-deterministic and may drift away from the target cardinality as $c$ approaches $r$. The Zipf distribution is used to model many big data phenomena, such as word frequency, website traffic, and city population. 

In the moving cluster dataset (MovC), the keys are chosen from a window that gradually slides. The  $i^{\text{\tiny th}}$ key is randomly selected the range $\left \lfloor{(c-W)i/r}\right \rfloor$ to $\left \lfloor{(c-W)i/r+W}\right \rfloor$, where the window size $W = 64$ and the cardinality $c$ is greater than the window size $(c >= W)$. The moving cluster dataset provides a gradual shift in data locality and is similar to workloads encountered in streaming or spatial applications.

% IDEA: For each dataset, calculate the number of duplicates for the top ranking key (with size and cardinality fixed to an average size). 

% In the self similar dataset, the keys follow the 80/20 rule. 
% Integers between 1...N.
% The first h•N integers get 1-h of the distribution.
% For example: if N = 25 and h= .10, then
%  80% of the weight goes to the first 5 integers.
%  and 64% of the weight goes to the first integer.
% code:
% long selfsimilar(long n, double h)
%  { return (1 + (int)
%  (N * pow((randf(),log(h)/log(1.0-h)))
%  );
%  }; 

==> design.tex <==

\section{Design considerations \sd{Can this be removed?}}
\label{sec:considerations} 


As the volume of data continuously grows, data scientists and analysts constantly look for simpler, quicker and more efficient ways to analyze and process this data.  Consider a scenario in which an analyst wants to perform some analytic tasks on a large  dataset, which does not fit in the main memory of the machine. Moreover, the data is stored as a raw text file (txt, csv or json). The three popular options 
% to perform this type of analysis 
include dedicated language-based frameworks, DBMSs, or big data frameworks. Next we discuss their trade-offs.

\textbf{Scalability of Dedicated Data Analytic Systems.} 
% The first option to process and analyze data is using a dedicated data analytic system. They 
These are typically based on language frameworks, such as R, MATLAB and Python. An important advantage of these approaches is that they typically have a large ecosystem of libraries supporting a diverse set of science tasks. 

In our scenario mentioned above, the data is relatively large and does not fit within the main memory of a machine. Hence, the analytic tasks may encounter severe performance issues or may not even complete. This issue was reported by previous data science benchmark studies such as in~\cite{Sanzu2017Watson}.  Until recently, 
% the way all dedicated data analytic systems worked was that all data was needed to be loaded into the main memory before performing an analysis task.
these frameworks required all data  to be loaded into the main memory before performing an analysis task. In recent times, several dedicated analytic systems have been extended with parallel computing libraries.  They automatically keep the data in the disk and load parts of the data into memory as needed for processing. An example
% of one of these libraries 
is Dask, 
% as mentioned in Section \ref{sec:microbenchmarkResult_scalability}. 
% Dask is the only framework, supporting Python data science library ecosystem, which we found that has the ability to scale out to a cluster of machines. 
however, it does not have SQL query support.  DaskDB extends Dask to support efficient \textit{in situ} query processing.

\textbf{The Challenge of ETL with DBMS.} 
%The second option is to use a DBMS.
Most modern DBMSs have data analytic capabilities and functionalities such as mentioned in Section \ref{related_in_database_ana}. Traditionally, database application developers need to create user-defined functions (UDF) for analytics, but a DBMS treats UDFs as black boxes with little or no optimizations.
% Depending on the DBMS, it is possible to execute UDFs written in R, Python, C, C++ or T-SQL languages. 
% The only way to interact with UDFs are through their input parameters and final output results.
%Further, they are often constrained in terms of the number and data types of its input and output. 
This results in them being difficult to debug and to incrementally develop~\cite{D'silva:2018:AIDA}. Moreover, the other major issue with a DBMS is the bottleneck involved with extracting, transforming and loading (ETL) the data into a DBMS. ETL is a time-consuming process and is not viable or necessary in many workflows. For example, only a subset of the data might be actually useful, and hence loading it into the database is a waste of time and resources. Also, with the data volume growing exponentially, a greater portion of the data for analysis is not being stored in databases. 


\textbf{Usability in Big Data System Frameworks.} The third option is to perform the analysis using a big data system framework. These frameworks can scale-up processing to multiple machines.
%(if machines are available and configured), partition the data into chunks and keep data in disk,  until chunks of the data are brought into main memory to process.
Furthermore, they enable automatically programming entire clusters with data parallelism and built-in fault tolerance. 
% Some popular frameworks include,  Spark \cite{SparkZaharia2010}, Hadoop~\cite{ShvachkoHadoop2010} and its SQL-based extension Hive~\cite{ ThusooHive2009}.
%, and often a combination of these frameworks are used in real-world applications. 
% Their programming interfaces include Java, Python, Scala, SQL (or a SQL-like language) and R,  and their functionalities include SQL querying capabilities, machine learning, streaming and graph libraries. 
The downside of these types of frameworks is that they often entail more complicated APIs and a steeper learning curve than the other two options.
%In general, big data frameworks are more complex, take  larger development effort and have comparatively lower usability. Furthermore,
% many programmers often have knowledge of high-level programming languages, but they
% programmers usually lack domain knowledge to use these frameworks effectively. 
Hence, 
% even though these frameworks may have popular data science language interfaces like Python and R, 
they require an analyst to use completely new APIs native to the big data framework. 
Furthermore, a vast body of data science applications exist that were written with language frameworks such as Anaconda Python or R. To run them within a  big data system, it will require rewriting these applications with new APIs. This is not a viable option in most cases.
% This results in an increase in time for non-experts to become proficient at using such a system. 
% We ran into this issue specifically while performing experimental evaluation with Spark. 
%% As we read the documentation, more was learned on how to optimize Sparks performance. 
% It took multiple iterations to find an optimal configuration by reading the documentation.  




==> tbd.tex <==
\section{Our approach}
\label{sec:tbd} 

Parallel aggregation involves deciding how to divide the work as well as how much data to share between the threads. 

Cieslewicz et al. \cite{cieslewicz2010automatic} discovered that sharing a common data structure between many cores does not perform well when the dataset contains heavy hitters (data items with high frequency). 

Some aggregation algorithms may split a group's tuples into separate data structures to allow for more efficient in-cache processing. These methods perform well for distributive and algebraic aggregation. Given the fact that holistic aggregation relies on having all of a group's tuples in one place, these methods cannot support exact holistic aggregation. 

Several popular parallel algorithms are as follows:
Independent: each thread creates a hash table on its own private set of data, and then the data from each of the tables is combined.
Shared: all threads access a single hash table, and use atomic instructions to safely update the table.
Hybrid: combine a single large global table with small private thread-local tables that are checked before checking the large table. 
Contention Detection: automatically detects frequently accessed data and clones it to reduce contention. There are two variants of this approach: in the local variant, the thread itself creates a clone in its local memory. In the global variant creates multiple global copies that are accessed by a balanced number of threads. 
Partition-and-Aggregate: partition the input based on group-by, and aggregate each group using a single thread. The partitions are arranged in a grid-like manner to avoid contention when writing the output.
PLAT: stands for Partition with a Local Aggregation Table. This algorithm extends partition-and-aggregate. Each thread has a local table to perform aggregation. One the table fills up, records that do not match the table are partitioned as in partition-and-aggregate.

\begin{table}
\caption{Aggregation}
\label{tab:freq}
\begin{tabular}{cccc}
\toprule
Aggregation Algorithm&Distributive&Algebraic&Holistic\\
\midrule
Shared & yes & yes & yes\\
Independent & yes & yes & no\\
Partition and Aggregate & yes & yes & yes \\
PLAT\cite{ye2011scalable} & yes & yes & no\\ 
Hybrid\cite{ye2011scalable} & yes & yes & no\\ 
Adaptive\cite{} & yes & yes & no\\
\bottomrule
\end{tabular}
\end{table}
